'Senator, We Sell Ads': Analysis of the 2016 Russian Facebook Ads Campaign

One of the key aspects of the United States democracy is free and fair elections that allow for a peaceful transfer of power from one President to the next. The 2016 US presidential election stands out due to suspected foreign influence before, during, and after the election. A significant portion of that suspected influence was carried out via social media. In this paper, we look specifically at 3,500 Facebook ads allegedly purchased by the Russian government. These ads were released on May 10, 2018 by the US Congress House Intelligence Committee. We analyzed the ads using natural language processing techniques to determine textual and semantic features associated with the most effective ones. We clustered the ads over time into the various campaigns and the labeled parties associated with them. We also studied the effectiveness of Ads on an individual, campaign and party basis. The most effective ads tend to have less positive sentiment, focus on past events and are more specific and personalized in nature. The more effective campaigns also show such similar characteristics. The campaigns' duration and promotion of the Ads suggest a desire to sow division rather than sway the election.

==> data.tex <==
\section{The Data}


The dataset comprises 3516 advertisements as released by the Data for Democracy organization \footnote{https://data.world/scottcame/us-house-psci-social-media-ads} in both csv and pdf file formats. Although the data is primarily obtained from the csv file, we also leverage the original pdf documents to account for the data unavailable or missing there. We now provide a brief statistical overview of the different features of the dataset. 

==> src/data_analytics.tex <==
\section{Data Analytics}

\textbf{Clicks and Impression counts:}
Clicks and impressions are important metrics to understand the outreach and efficacy of the advertisement. Clicks, or link clicks, quantify the number of people who have clicked on the ad and was redirected to the particular landing-page. Impressions refer to the total number of times the advertisement has been shown. It differs from  Reach which reflects instead the  number of individual people who have seen the ad. 

\begin{figure}[htb]   
	\vspace{-1.0cm}
	\centering
    
    \subfloat[Impressions vs Ad]
    {
    \includegraphics[width=0.33\textwidth]{Figures/impressions_hist.png}
    \label{impressions-ad-dist}
	}
    \subfloat[Clicks vs Ad\label{clicks-ad-dist}]
    {
    \includegraphics[width=0.33\textwidth]{Figures/clicks_hist.png}
	}
    \subfloat[Correlation between clicks and impressions \label{clk_imp_correlation}]
    {
    \includegraphics[width=0.3\textwidth]{Figures/clk_imp_rel.png}
	}
    \vspace{-2mm}
    \caption{Distribution of Clicks and Impressions}
    \label{fig:clks-imp-dist}
    \vspace{-7mm}
\end{figure}

We present the distribution of impressions and clicks for the FB ads in \ref{fig:clks-imp-dist}(a) and \ref{fig:clks-imp-dist} (b) respectively. It is clearly evident that a majority of ads have attained sufficient outreach and popularity. We also see there exists a strong correlation (r=0.8927) between the impressions and clicks as seen in the Figure \ref{fig:clks-imp-dist}(c). 

\textbf{Target Age groups:}
We observe that a huge fraction of the ads are targeted to the younger age group as seen in \ref{fig:age-date-dist} (a). 

\begin{figure}[thb]
	% Center the figure.
    \vspace{-10mm}
	\centering
    
    \subfloat[Age group targeted by the ads.]
    {
    \includegraphics[height=0.3\textwidth,width=0.5\columnwidth]{Figures/target_age.png}
%     \includegraphics[width=0.33\textwidth]{Figures/impressions_hist.png}
    \label{target-age-dist}
	}
    \subfloat[Timeline of the advertisements \label{timeline}]
    {
    \includegraphics[width=0.6\textwidth]{Figures/init_date_series.png}
	}
    
    \caption{Age-wise and timeline distribution of the advertisements}
	\label{fig:age-date-dist}
	\vspace{-10mm}
\end{figure}

\textbf{Time-line analysis:}
We also observe the specific time-line when the advertisements were posted as shown in \ref{fig:age-date-dist}(b). Although several advertisements were floated during the election period of 2016, a substantial portion was posted both prior to and after the elections.

\textbf{Language Distribution}
A majority of the advertisements (54.29\%) did not have a valid language field. To circumvent this predicament, we leveraged the language detector library of TextBlob \footnote{http://textblob.readthedocs.io/en/dev/}, which is powered by the Google Translate API to identify the language of the advertisement text.\footnote{https://cloud.google.com/translate/docs/}. 
Unsurprisingly, almost all the advertisements (98.349\%) are conveyed in English, with small fractions in Arabic (0.341\%), Spanish (0.284\%) and other languages (0.142\%, comprising Italian, Hindi, Portugese, etc). There are also 32 ADs whose language could not be identified due to absence of any text in the advertisement. Overall, it is evident that most of the ads were targeted towards the English speaking population, which comprises 91.4\% of the American population. \footnote{http://blog.languageline.com/limited-english-proficient-census}


\textbf{Landing Page Analysis}
We present here an overview of the common landing pages that had posted these advertisements. Surprisingly, we found several pages which had posted  advertisements on more than one occasion. 
%We depict the frequency distribution of ads of different pages in the figure \ref{fig:landing_page}.
We illustrate some popular pages in the table \ref{tab:landing_page}.

\begin{table}[tb]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
Landing Page & \#Ads &Landing Page &\#Ads  \\  \hline

% https://www.facebook.com/Black-Matters-1579673598947501/&	260 & https://www.facebook.com/patriototus&	83\\
% https://www.facebook.com/blackmattersus.mvmnt/&	232 & https://www.facebook.com/Woke-Blacks-294234600956431/&	81\\
% https://www.facebook.com/brownunitedfront/&	204 &https://www.facebook.com/savethe2a/&	68\\
% https://www.facebook.com/WilliamsandKalvin/&	170 & https://www.facebook.com/Stop-Al-896610653786585/&	63\\
% https://www.facebook.com/blacktivists/&	159 & https://www.facebook.com/WilliamsKalvin-788980617892144/&	63\\
% https://www.facebook.com/Memopolis-450474615151098/&	154 & https://www.facebook.com/PanAfrootsmove/&	60\\
% https://www.facebook.com/Blacktivist-128371547505950/&	132 & https://www.facebook.com/blackmattersus/&	59\\
% https://www.facebook.com/Dont-Shoot-1157233400960126/&	109 &https://www.facebook.com/MuslimAmerica/&	54\\
% https://musicfb.info/&	107 & https://www.facebook.com/stoptherefugees/&	50\\
% https://www.facebook.com/LGBT-United-839497472793277/&	95 & https://www.facebook.com/StopAllInvaders&	49\\

https://www.facebook.com/blackmattersus/&	291 & https://www.facebook.com/LGBT-United/& 95\\
https://www.facebook.com/Black-Matters-/&	260  &https://www.facebook.com/patriototus&	83\\
https://www.facebook.com/WilliamsandKalvin/& 233 & https://www.facebook.com/Woke-Blacks-/&	81\\
https://www.facebook.com/brownunitedfront/&	204 &https://www.facebook.com/savethe2a/&	68\\
https://www.facebook.com/blacktivists/&	159 &  https://www.facebook.com/Stop-Al/&	63\\
https://www.facebook.com/Memopolis/&	154 & https://www.facebook.com/PanAfrootsmove/&	60\\
https://www.facebook.com/Blacktivist/&	132 & https://www.facebook.com/MuslimAmerica/&	54\\
https://www.facebook.com/Dont-Shoot/&	109 & https://www.facebook.com/stoptherefugees/&	50\\
https://musicfb.info/&	107 & https://www.facebook.com/StopAllInvaders&	49\\
\hline
\end{tabular}}
\caption{Some frequent landing pages}
\label{tab:landing_page}
\vspace*{-8mm}
\end{table}


\textbf{Gender-wise Distribution}
A majority of the ads(95.762\%) did not have a valid gender field, while the ads directed towards Males and Females accounted for 3.100\% and 1.137\% respectively. The frequent interests associated with the advertisements which are directed towards a particular gender are shown in Table \ref{tab:gender-interests}. We observe that the ads directed exclusively towards males talks about gun rights and the second amendment, the ones directed exclusively towards women had light-hearted topics like music and funny pictures, while the rest referred to serious issues that affected both namely racism, police accountability. 

\vspace{-0.4cm}
\begin{table}[htb]
\centering
\resizebox{0.75\textwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline

Males&Females&Both\\ \hline
gun rights& music& african-american history\\
anything about guns& funny pictures& african-american civil\\
&&rights movement (1954-68)\\
guns and patriots& funny pics& martin luther king jr \\
guns & lol& malcolm(x) \\
free music & free software& la raza\\	
national rifle association	& funny photo's & cop block \\
2nd amendment& black economic empowerment & chicano movement\\
& interest expansion	&\\
\hline
\end{tabular}}
\caption{Common interests of gender-directed ads}
\label{tab:gender-interests}
\vspace*{-15mm}
\end{table}

\textbf{Currency Analysis}
Facebook \footnote{https://www.facebook.com/business/products/ads} enables businesses and entrepreneurs to market their ideas and specify the corresponding target audience for a requisite price. Higher the cost of the advertisements, greater is the outreach. Consequently, it is not surprising to observe that a majority of these advertisements (69.94\%) were paid. Apart from 4 isolated ads, the currency for facilitating this transaction was in Russian Rubles (RUB). The total cost involved/ expended was a staggering 4,912,799.70 rubles, which amounts to \$78,604 USD.
We represent the frequency distribution of the money spent on the ads in Figure \ref{fig:currency_ads} (a) and acknowledge that a significant portion (43.714\%) of them have paid between 100-1000 rubles. Similarly, in Figure \ref{fig:currency_ads} (b), we observe that even after the completion of the 2016 elections, money still poured into the ads, indicating that the primary objective of the ads might not have been to influence the electoral results. 

\begin{figure}[thb]
	% Center the figure.
	\centering
    
    \subfloat[Frequency Distribution of money spent]
    {
    \includegraphics[height=0.35\textwidth,width=0.5\columnwidth]{Figures/currency_ads.png}
	}
    \subfloat[Temporal distribution of money spent ]
    {
    \includegraphics[height=0.35\textwidth, width =0.5\textwidth]{Figures/cdf_curr.png}
	}
    \caption{Money spent on purchasing the Russian ads}
    \label{fig:currency_ads}
\vspace{-5mm}
\end{figure}

Since the aim of targeted promotion is to popularize ads and increase its outreach, it is unsurprising to observe a decent correlation between the number of clicks / impressions and the money spent on the ad (r=0.615 and r=0.592 respectively). 







\textbf{Textual and Image Analysis}
A significant proportion of the advertisements have textual and image information embedded in them (99.08\% and 88.51\% respectively). We leverage this information to analyze the differences in effectiveness between the high and low performance ads, which we outline in the next section. 

\textbf{Other Metadata}
Some of the advertisements have other metadata information associated with them like, 
political leaning (1.649\%), behaviors(9.812\%), custom audience (0.853\%), %excluded connections (26.9\%), 
people who match(12.116\%) etc. Although essential, such information is present only in small proportions. The percentages indicate the proportion of ads which had the corresponding valid metadata information. Consequently, we disregarded this corresponding information. 















% The interesting phenomena for each of these three metrics is that they are not correlated with the cost. The Pearson coefficient of correlation (r) for CTR, CPC and CPM is 0.0036 , 0.0164 and 0.0252 respectively. 
% Consequently, a high CTR value and low CPC (or CPM) value implies that the ad was sufficiently creative or compelling to garner a high acceptance.


